SuperFedNAS: Cost-Efficient Federated Neural Architecture Search for On-Device Inference

Neural Architecture Search (NAS) for Federated Learning (FL) is an emerging field. It automates the design and training of Deep Neural Networks (DNNs) when data cannot be centralized due to privacy, communication costs, or regulatory restrictions. Recent federated NAS methods not only reduce manual effort but also help achieve higher accuracy than traditional FL methods like FedAvg. Despite the success, existing federated NAS methods still fall short in satisfying diverse deployment targets common in on-device inference like hardware, latency budgets, or variable battery levels. Most federated NAS methods search for only a limited range of neuro-architectural patterns, repeat them in a DNN, thereby restricting achievable performance. Moreover, these methods incur prohibitive training costs to satisfy deployment targets. They perform the training and search of DNN architectures repeatedly for each case. SuperFedNAS addresses these challenges by decoupling the training and search in federated NAS. SuperFedNAS co-trains a large number of diverse DNN architectures contained inside one supernet in the FL setting. Post-training, clients perform NAS locally to find specialized DNNs by extracting different parts of the trained supernet with no additional training. SuperFedNAS takes O(1) (instead of O(N)) cost to find specialized DNN architectures in FL for any N deployment targets. As part of SuperFedNAS, we introduce MaxNet - a novel FL training algorithm that performs multi-objective federated optimization of a large number of DNN architectures ($\approx 5*10^8$) under different client data distributions. Overall, SuperFedNAS achieves upto 37.7% higher accuracy for the same MACs or upto 8.13x reduction in MACs for the same accuracy than existing federated NAS methods.

==> 00-abstract.tex <==
Neural Architecture Search (NAS) for Federated Learning (FL) is an emerging field. It automates the design and training of Deep Neural Networks (DNNs) when data cannot be centralized due to privacy, communication costs, and regulatory
restrictions. Recent federated NAS methods not only reduce manual effort but also provide more accuracy than traditional FL methods like FedAvg , which use predefined DNN architectures. 
% However, existing federated NAS methods incur a huge communication cost and provide sub-optimal architectures when on-device inference metrics like latency/FLOPs are considered. 
% However, most state-of-the-art federated NAS methods follow a multi-stage FL training that often leads to
high communication costs. Furthermore, these methods severely restrict DNN architecture diversity and thereby provide sub-optimal architectures when on-device inference metrics like latency/FLOPs are considered.
% \payman{To me this is a vague statement. We need to list the tangible problems with a simple language here.}
% \payman{do you want to mention that current method provide a single optimal point which may not be useful in practice since the device characteristics are changing dynamically during deployment}
To address these challenges, we propose \proposedfed: a one-stage federated NAS method that jointly trains a rich diversity of DNN architectures (subnets) contained inside one supernet. 
Clients can then perform NAS locally to find
% Post the FL training stage, clients perform NAS locally to find
specialized DNNs by extracting different parts of the trained supernet with no additional training. 
\proposedfed takes $O(1)$ (instead of $O(k)$) cost to find specialized DNN architectures in FL for any $k$ hardware/latency targets. As part of \proposedfed, we introduce \proposedTraining---a novel FL training algorithm that performs joint federated optimization of a large number of DNN architectures cost-efficiently. 
% \alexey{one of the reviewers complained about us making a big deal about this huge number of architectures mentioned below. }
\proposedTraining trains a family of  $\approx 5*10^8$ diverse subnets with up to $9.34$x computational and $10.94$x communication cost reduction compared to state-of-the-art. Overall, FedNasOdin achieves up 
 to $15$\% higher accuracy for the same FLOPs or upto $18.52$x reduction in FLOPs for the same accuracy than existing federated NAS methods.
 % \alexey{nice finish.} 

% \proposedfed's training stage jointly trains  
% SOTA problems cited: high cost and suboptimal latency/FLOPs for the same acc.

==> 01-intro.tex <==
Federated Learning (FL) is increasingly used in numerous applications like GBoard \cite{gboard}, Apple's Siri \cite{siri}, pharmaceutical discovery \cite{fl_pharma}, medical imaging \cite{medical-imaging}, health record mining \cite{fed_ehr1}, and recommendation systems \cite{fl_recommending}. In federated learning, a large number of clients collaboratively participate in a distributed training of a deep neural network (DNN) while keeping their data private \cite{fedavg, fed_distill, fedma, scaffold, fed_strategy}. FL offers three key benefits:
a) smaller communication costs,
b) massive parallelism, and
c) no data sharing \payman{Maybe privacy preserving}. Despite the success, most FL works still use manually designed predefined DNN architectures. This may lead to sub-optimal accuracy, especially in the federated context when the data generated by clients remains invisible the model developers \cite{fl_challenges} and makes the manual designing of DNN architectures significantly challenging. Rather, there is a need to automatically design and train optimal DNN architectures in FL for better accuracy.
\payman{here we introduce the first problem of SOTA. However, there are issues:
1- I think the first problem should be the biggest problem. So, the reviewer says wow. right problem to work on it.
2- Next paragraph you forget about problems and talk about automation. That leads to discontinuity of speech. We need to talk about 1- why do we need NASFL 2- what are the problems of SOTA and 3- suggested problems in-order}\alind{how about now?}
To automate the design and training of DNNs in FL, recent works propose neural architecture search (NAS) methods for FL \cite{fednas, fedpnas}. The goal of such methods is then to find the most accurate DNN architecture globally \cite{fednas} \alind{or locally personalized to each client \cite{fedpnas}}. They perform federated NAS and provide more accuracy than traditional FL methods like FedAvg \cite{fedavg} that use a predefined DNN architecture. \payman{Need a lot of citation here}
% More recently, many works propose NAS-based methods for personalized FL \cite{fedpnas} and provide personalized DNN architectures for clients. 
Such developments in federated NAS methods hold great promise to provide efficient DNNs adapted to clients' data by design.

However, existing federated NAS methods fail to provide optimal DNN architectures for efficient on-device inference when different deployment scenarios like latency/FLOP budgets, hardware, etc. are considered. 
% This is multiple latency/FLOP targets which is crucial for efficient deployment for on-device inference. 
This is due to the following limitations:
\begin{displayquote}
\end{displayquote}

However, existing federated NAS methods \cite{fednas} incur a huge communication cost (\textbf{C1}). The huge communication cost (\textbf{C1}) comes due to the expensive two-staged federated learning process \cite{fednas} where, in the first stage (\textit{searching}), multiple DNN architectures are simultaneously searched and trained by clients. In the second stage (\textit{evaluation}), the best-performing DNN architecture from the first stage is trained using FedAvg \cite{fedavg}. 
% \\
Moreover, the federated NAS methods don't provide optimal DNN architectures when on-device inference metrics like latency/FLOPs are taken into consideration (\textbf{C2}).
\payman{what is the metric for not being optimal? size? latency? diversity? what? we need to be clear on this and mention it.}
This is because these methods severely restrict DNN architecture diversity and thereby harm performance. For instance, FedNAS \cite{fednas} searches for only a few DNN architectures and then repeatedly stacks the same pattern limiting the layer diversity. FedPNAS \cite{fedpnas}
keeps a large base component the same among all DNN architectures and only allows the architecture to differ in small personalized components. 

\payman {We need to quantify C1 and C2 and provide some results . That can be like motivational plots. Without them, it seems very high level statements. Also we need to say where does this communication cost come from?  Who identifies huge? what is a threshold for being huge? Also, I would suggest not using emotional words like huge. It may hurt reviewers. we can say high instead of huge.
To me the most selling point part of the paper is to convince a reviewer you are working on an important problem}

To solve the aforementioned challenges (\textbf{C1}, \textbf{C2}), we propose \proposedfed : a one-stage federated NAS method (for \textbf{C1}) that trains a rich diversity of DNN architectures for efficient on-device inference (for \textbf{C2}). \proposedfed flexibly supports different
depths (per stage) and widths (per layer) among DNN architectures (subnets) contained inside a single supernet. During on-device inference, specialized DNN architectures are used by selecting different parts of the supernet without retraining. Inspired by recent advances in centralized NAS methods \cite{ofa}, \proposedfed only has one FL training stage that jointly trains a large number of subnets as a part of the supernet. Post the FL training stage, the trained supernet is provided to each client to perform NAS locally. The local NAS doesn't require any additional training of subnets and thereby has a negligible cost. Given the target hardware and latency constraint, local NAS finds specialized DNN architectures (subnets) using predictor-guided search \cite{predictor_guided_search}. Overall, \proposedfed reduces the cost to find specialized DNN architectures in FL for $k$ different hardware/latency targets to $O(1)$, whereas prior federated NAS methods \cite{fednas} remain $O(k)$ (prohibitively expensive and don't solve \textbf{C1}) as they need to train and search repeatedly for each on-device inference deployment target.

% \alind{Continue and talk about why training multiple DNN archs is non-trivial in FL}
However, training the supernet in a federated setting is a non-trivial task, as it requires joint federated optimization of the shared weights to maintain the accuracy of a large number of subnets across clients. \payman{To me joint here is not clearly defined. joint of what and what?!} 
% We find (and later show) that 
To make things worse, directly applying centralized supernet training methods like Progressive Shrinking (PS) \cite{ofa} to the federated setting doesn't solve the challenges \textbf{C1, C2}. First, PS introduces a multi-stage approach to training supernets and gradually relaxes the search space to add smaller subnets to training. If applied to the FL setting, the multi-stage supernet training approach increases the communication cost significantly and doesn't solve \textbf{C1} \payman{I prefer saying due to  A, B,C} similar to existing federated NAS methods. Furthermore, we find that applying PS in FL for joint federated optimization of many subnets often leads to slow convergence as different subnets interfere with each other. \payman{ I think we need to provide some results for this. It would be appreciated by reviewers} This interference results in sub-optimal accuracy of subnets and fails to provide optimal DNN architectures, and as a result, doesn't solve \textbf{C2}.

To efficiently perform joint federated optimization of a large number of subnets, we propose \proposedTraining: a training algorithm for \proposedfed that trains supernets in one FL training stage (for \textbf{C1}) and reduces interference (for \textbf{C2}). First, \proposedTraining decides \textit{which} individual subnets are distributed for training on participating clients and \textit{when} (\textit{subnet distribution}). \proposedTraining's subnet distribution optimizes both the lower bound (smallest subnet) and upper bound (largest subnet) to achieve higher accuracy across all subnets in between.
Second, 
since all subnets partially share their weights,  \proposedTraining introduces a novel shared model weight aggregation mechanism that mitigates interference. To summarize, our contributions are as follows: 
\begin{tightitemize}
\item \proposedfed: A one-stage federated NAS method that trains a rich diversity of DNN architectures for efficient on-device inference.
\item \proposedfed produces specialized DNN architectures for $k$ hardware/latency targets in on-device inference with O(1) cost. Post the training stage of \proposedfed the DNN architectures don't require any additional training.
\item \proposedTraining: An FL training algorithm that performs joint federated optimization of a large number of DNN architectures in the supernet and reduces interference. 
% It reduces interference among the subnets by innovating subnet distribution and aggregation and enables dynamic prioritization of contributed model weights.
\end{tightitemize}
\payman{Maybe enabling the algorithm for text dataset can also be a valid contribution.}

\proposedfed outperforms existing federated NAS methods across multiple vision (CIFAR10/100, CINIC-10) and text datasets (Shakespeare dataset derived from LEAF~\cite{leaf}), degrees of statistical heterogeneity, and client participation probability. It achieves upto $15$\% higher accuracy for the same FLOPs or the same accuracy with $18.52$x reduction in FLOPs than existing federated NAS methods. \proposedTraining trains a family of  $\approx 5*10^8$ diverse subnets with upto $9.34$x computational and $10.94$x communication cost reduction compared to state-of-the-art.

\payman{My suggestion is to add motivation/background section and add motivational plots such as high communication cost and interference there. Plus we can talk more extensively about where this communication cost come from and what is the impact of it. We can talk about why we need weight sharing method.  }
% close to an order of magnitude lower computational (9.43x) and communication (10.94x) cost compared to training only 9 independent subnetworks with \fedavg--- the cost reduction achieved with no accuracy loss.
% IHowever, joint federated optimization of a large number of DNN architectures 
% such methods need to search for only a few architectural motifs and then
% repeatedly stack the same pattern, which restricts the block diversity and thereby harms performance.

% as they simultaneously train and search DNN architectures. Due to the simultaneous search and training of DNNs, these federated NAS methods become two-staged \cite{fednas} severely increasing the communication cost. In the first stage, the methods perform  
% remain prohibitively expensive  and fail to provide DNNs specialized for inference in client's device.


% the communication cost of such methods remains prohibitively expensive as these methods perform a heavy operation of simultaneous search and training of multiple DNN architectures. We argue that this operation often leads to increased communication costs due to two drawbacks. First, the simultaneous search and training of DNN architectures leads to sub-optimal weights
% to produce optimal DNNs trained in FL. 
% We argue that the fundamental reason for the high communication cost of NAS methods in FL is  It  
% increases their communication cost due to reasons.

% For instance, FedNAS \cite{fednas} simultaneously searches and trains multiple DNN architectures locally in each client and then later trains the best-performing architecture using FedAvg. These stages increase the communication cost of FedNAS.
% all these methods perform a heavy operation of simultaneously training and searching the DNN architectures 

==> Figs/code/client_class_distribution.tex <==
\begin{figure*}[h!]
	\centering
	\begin{subfigure}[b]{0.3\textwidth}

        \includegraphics[width=1\textwidth]{Figs/Alpha100_Client_Class_Distribution.pdf}
	    \caption{
		     non-iid=100.
		}
	\end{subfigure}
	\begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=1\textwidth]{Figs/Alpha1_Client_Class_Distribution.pdf}
	    \caption{
		    non-iid=1.
		}
	\end{subfigure}
	\begin{subfigure}[b]{0.3\textwidth}
        \includegraphics[width=1\textwidth]{Figs/Alpha0_1_Client_Class_Distribution.pdf}
	    \caption{
		    non-iid=0.1.
		}
	\end{subfigure}
   
    \caption{
	   \small \textbf{Non-i.i.d Degree}. Client class distribution visualization across different non-iid$=\{100, 1, 0.1\}$ values. Showing visualizations for CIFAR10 dataset partitioned using Drichlet distribution among 20 clients.
	}
	 \label{fig:client_class_distribution}
\end{figure*}

==> Figs/code/dnn_arch_space.tex <==
% \begin{figure*}[t!]
%     \centering
%     \vspace{-3mm}{{\includegraphics[width=0.6\columnwidth]{Figs/WSConcept.pdf}}}
%     \caption{Weigh Sharing Concept} 
%     \label{fig:WSConcept}
%     \vspace{-2ex}
% \end{figure*}

==> Figs/code/nas_results.tex <==
\begin{figure*}[t]
% \vspace{-0.7cm}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Figs/GPU_NAS_Pareto.pdf} % Adjust the height as needed
        \caption{RTX 2080Ti}
        \label{fig:nas_pareto:cpu}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Figs/CPU_NAS_Pareto.pdf}
        \caption{AMD CPU}
        \label{ffig:nas_pareto:gpu}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.37\textwidth}
    %     \includegraphics[width=\textwidth]{Figs/FedNASODIN-Approach.pdf}
    %     \caption{Naive Single-Stage Supernet FL}
    %     \label{fig:single_stage}
    % \end{subfigure}
    % \vspace{-2ex}
    \caption{\small \textbf{\proposedfed's Pareto-Optimal Subnets for Target Hardware}  \proposedfed's search stage trains and searches for Pareto optimal subnets for different target hardware compared manually trained DNNs (using scaling rule \cite{efficient_net}) with FedAvg \cite{fedavg}.}  
    % architecture (with 85.25\% accuracy) for 112 ms latency target on AMD CPU and wide/deep DNN architecture (with 91.56\% accuracy) for 18.2 ms latency target on RTX 2080Ti GPU.} 
    \label{fig:nas_pareto}
     % \vspace{-0.7cm}
     % \vspace{-2ex}
\end{figure*}


==> algs/maxnet.tex <==
\begin{algorithm}[htb]
\footnotesize
   \caption{\small \proposedTraining's Supernet FL-Training}
   \label{alg:maxnet}
\begin{algorithmic}[1]\footnotesize

 \STATE Initialize $W$ \algorithmiccomment{Supernet Weights}
 \STATE CNT$_{\alpha_{max}}$,CNT$_{\alpha_{min}}$ = \{k:0 for $k \in \kappa$\}\algorithmiccomment{tracker for min/max subnet assignment}
 \STATE Initialize $\beta$\algorithmiccomment{Initial value for Maxnet's hyper-param}

  \FOR{round t = 1,2, ... T}
   \STATE $\kappa_t \leftarrow$ random set of $max(C\cdot K, 1)$  clients ($\kappa_t \subseteq \kappa$)\algorithmiccomment{randomly pick C.K clients}
   \STATE k$_{{max}}$ = argmin$_{k \in \kappa_t}$ CNT$_{\alpha_{max}}$[k] \algorithmiccomment{client with least assignment of max subnet}
   \STATE k$_{{min}}$ = argmin$_{k \in \kappa_t}$ CNT$_{\alpha_{min}}$[k] \algorithmiccomment{client with least assignment of min subnet} 
   \STATE $h_t =$ ($k_{{max}}$,$\mathcal{G}(W_t, \alpha_{max})$) $\cup$ ($k_{{min}}$,$\mathcal{G}(W_t, \alpha_{min})$)\algorithmiccomment{assign max,min subnets}
   \STATE $h_t =$\{(k,$\mathcal{G}(W_t, \alpha_k)$): $k \in \kappa_t \setminus \{k_{{min}},k_{{max}}\}$ \& $\alpha_k \in \mathcal{U}(\mathcal{A})$\}  \algorithmiccomment{randomly assign subnets to rest of the clients}
   
   \FOR{client $k \in \kappa_t$}
    \STATE $w^{t}_k \leftarrow h_t(k)$ \algorithmiccomment{clients only receive subnet weights}
    % , $w^{t}_{k}  \leftarrow \mathcal{G}(W_t, \alpha^{t}_k)$
   \STATE $w^{t+1}_{k} \leftarrow$  ClientUpdate(k ,$w^{t}_{k}$) \algorithmiccomment{train subnet locally}
  \ENDFOR
  % \STATE $W^{t+1}=$ $\frac{\beta. \frac{n_{k_{\alpha_{max}}}{} .w^{t+1}_{k_{\alpha_{max}}} + (1-\beta).\sum_{k \in \kappa_t \setminus \{k_{\alpha_{max}}\} }   }  }{}$
  \STATE  $W^{t+1}=$ $\frac{ \beta_t. \frac{n_{k_{{max}}}}{n}. w^{t+1}_{k_{{max}}}   + (1-\beta_t).\sum_{k \in \kappa_t \setminus \{k_{{max}}\} } \frac{n_k}{n}.w^{t+1}_k }{\beta_t. |w^{t+1}_{k_{{max}}}|   + (1-\beta_t).\sum_{k \in \kappa_t \setminus \{k_{{max}}\} } .|w^{t+1}_k| }$ \algorithmiccomment{wt. cardinal averaging}
  \STATE CNT$_{\alpha_{max}}$[k$_{{max}}$] += 1, CNT$_{\alpha_{min}}$[k$_{{min}}$] += 1 \algorithmiccomment{update counters}
  \STATE $\beta_{t+1}$ = decay($\beta_t$, t) \algorithmiccomment{decay $\beta$}
  % \STATE $W^{t+1} = \frac{\beta.\frac{n_{k_{\alpha_{max}}}}{n}.w^{t+1}_{k_{\alpha_{max}}}+ (1-\beta).\sum_{k \in \kappa_t\setminus\{k_{\alpha_{max}}\} w^{t+1}_{k_{\alpha_{max}}}
  % + (1-\beta).k_{\alpha_{max}}\}}w^{t+1}_{k}}{\sum_{k \in \kappa_t\setminus\{k_{\alpha_{max}}\}}|w^{t+1}_{k}|}$ \algorithmiccomment{cardinal averaging of supernet weights}
 % \STATE $W^{0} \leftarrow$ zeros($W_{t}$) \algorithmiccomment{shared-param avg by overlap cardinality}
 % \STATE $W_{sum}  \leftarrow \sum_{k\in S_t} n_k*\mathcal{M}(W^{0},\;arch^{k}_t ,\;w^{k}_{t+1})$
 % \STATE $W_{sum} \leftarrow $  replace\_zeros($W_{sum}$, $W_t$) %
 % \STATE $W_{cnt} \leftarrow \sum_{k\in S_t} \mathcal{M}(W^{0}, arch^{k}_t , n_k*ones(w^{k}_{t+1}))$
 % \STATE $W_{cnt} \leftarrow $  replace\_zeros($W_{cnt}$, $1$) %
 % \STATE $W_{t+1} \leftarrow \frac{W_{sum}}{W_{cnt}}$
\ENDFOR
\end{algorithmic}
\end{algorithm}
% \vspace{-0.1in}




==> algs/maxnet_parameter_averaging.tex <==
\begin{algorithm}[H]
\footnotesize
   \caption{\small
    \spatioTempHeuristic's Shared-Param Averaging For Round $t$ after clients' local updates
    }
   \label{alg:maxnet_shared_param_averaging}
   % \vspace{-0.5in}
\begin{algorithmic}[1]\footnotesize
\STATE {\bfseries Input:} Client j ($j\in S_t$) which has been assigned the largest subnetwork at $t^{th} round$ ($\mathcal{H}(t)(j) = arch_M$), $S_t$ is set of randomly sampled clients $t^{th}$ round 
\STATE $\beta_{t} = decay(\beta_0, t)$
 \STATE $W^{0} \leftarrow$ zeros($W_{t}$)
 \STATE $W_{sum}  \leftarrow \sum\limits_{k\in S_t \setminus j} \frac{(1-\beta_t)}{|S_t| - 1}*n_k*\mathcal{M}(W^{0},\;arch^{k}_t ,\;w^{k}_{t+1})$
 \STATE $W_{sum}  \mathrel{+}= \beta_t*n_j*\mathcal{M}(W^{0},\;arch_M ,\;w^{j}_{t+1})$ \algorithmiccomment{largest subnet}
 \STATE $W_{sum} \leftarrow $  replace\_zeros($W_{sum}$, $W_t$) \algorithmiccomment{no overlaps}
 \STATE $W_{cnt} \leftarrow \sum\limits_{k\in S_t \setminus j} \mathcal{M}(W^{0}, arch^{k}_t , \frac{(1-\beta_t)}{|S_t| - 1}*n_k*ones(w^{k}_{t+1}))$
 \STATE $W_{cnt}\mathrel{+}= \beta_t*\mathcal{M}(W^{0},arch_M ,n_j*ones(w^{j}_{t+1}))$
 \STATE $W_{cnt} \leftarrow $  replace\_zeros($W_{cnt}$, $1$) \algorithmiccomment{no overlaps}
 \STATE $W_{t+1} \leftarrow \frac{W_{sum}}{W_{cnt}}$
\end{algorithmic}
\end{algorithm}



==> algs/ps_fl.tex <==
\begin{algorithm}[htb]
\footnotesize
   \caption{\small Multi-Stage Supernet FL-Training}
   \label{alg:ps_fl}
\begin{algorithmic}[1]\footnotesize

 \STATE Initialize $W$ \algorithmiccomment{Supernet Weights}
  \FOR{phase p in \{depth, width\}}
  \FOR{round t = 1,2, ... T$_{p}$}
  
   \STATE $\kappa_t \leftarrow$ random set of $max(C\cdot K, 1)$  clients ($\kappa_t \subseteq \kappa$)\algorithmiccomment{randomly pick C.K clients}
%    % \STATE $h_t =$\{(k,$\mathcal{G}(W_t, \alpha_k)$): $k \in \kappa_t$ \& $\alpha_k \in \mathcal{U}(\mathcal{A})$\}  \algorithmiccomment{randomly assign subnets to clients}
   
   \FOR{client $k \in \kappa_t$}
    % \STATE $w^{t}_k \leftarrow h_t(k)$ \algorithmiccomment{clients only receive subnet weights}
%     % , $w^{t}_{k}  \leftarrow \mathcal{G}(W_t, \alpha^{t}_k)$
    \FOR{(x,y) in minibatch($D_k$)}
    \FOR{$\alpha$ in PS-Sample($\mathcal{A}$,p)} 
    % \STATE loss = crossEntropy(forward(x,$\mathcal{G}(W_t, \alpha)$)) \algorithmiccomment{loss on subnet}
    \STATE crossEntropy(forward(x,$\mathcal{G}(W_t, \alpha)$)) 
    \STATE loss.backward() \algorithmiccomment{ gradients of subnet sampled based on phase}
    \ENDFOR
   % \ENDFOR
   \STATE $W^{t+1}_k \rightarrow$ optimizer.step() \algorithmiccomment{clients train supernet locally using PS \cite{ofa}}
  \ENDFOR
  \STATE $W^{t+1} = \frac{1}{|C.K|}\sum_{k \in \kappa_t} \frac{n_k}{n}.W^{t+1}_{k}$ \algorithmiccomment{FedAvg\cite{fedavg} aggregation of supernet weights}
  \ENDFOR
%  % \STATE $W^{0} \leftarrow$ zeros($W_{t}$) \algorithmiccomment{shared-param avg by overlap cardinality}
%  % \STATE $W_{sum}  \leftarrow \sum_{k\in S_t} n_k*\mathcal{M}(W^{0},\;arch^{k}_t ,\;w^{k}_{t+1})$
%  % \STATE $W_{sum} \leftarrow $  replace\_zeros($W_{sum}$, $W_t$) %
%  % \STATE $W_{cnt} \leftarrow \sum_{k\in S_t} \mathcal{M}(W^{0}, arch^{k}_t , n_k*ones(w^{k}_{t+1}))$
%  % \STATE $W_{cnt} \leftarrow $  replace\_zeros($W_{cnt}$, $1$) %
%  % \STATE $W_{t+1} \leftarrow \frac{W_{sum}}{W_{cnt}}$
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}
% \vspace{-0.1in}




==> algs/two_algos.tex <==
\noindent
\begin{minipage}{\textwidth}
  \centering
  \begin{minipage}{.47\textwidth}
    \centering
    \input{algs/weight_shared_training_algorithm}
  \end{minipage}
  \begin{minipage}{.52\textwidth}
    \centering
    \input{algs/maxnet_parameter_averaging}
  \end{minipage}
\end{minipage}

==> algs/weight_shared_training_algorithm.tex <==
\begin{algorithm}[htb]
\footnotesize
   \caption{\small Single-Stage Supernet FL-Training}
   \label{alg:single_stage}
\begin{algorithmic}[1]\footnotesize

 \STATE Initialize $W$ \algorithmiccomment{Supernet Weights}

  \FOR{round t = 1,2, ... T}
   \STATE $\kappa_t \leftarrow$ random set of $max(C\cdot K, 1)$  clients ($\kappa_t \subseteq \kappa$)\algorithmiccomment{randomly pick C.K clients}
   \STATE $h_t =$\{(k,$\mathcal{G}(W_t, \alpha_k)$): $k \in \kappa_t$ \& $\alpha_k \in \mathcal{U}(\mathcal{A})$\}  \algorithmiccomment{randomly assign subnets to clients}
   
   \FOR{client $k \in \kappa_t$}
    \STATE $w^{t}_k \leftarrow h_t(k)$ \algorithmiccomment{clients only receive subnet weights}
    % , $w^{t}_{k}  \leftarrow \mathcal{G}(W_t, \alpha^{t}_k)$
   \STATE $w^{t+1}_{k} \leftarrow$  ClientUpdate(k ,$w^{t}_{k}$) \algorithmiccomment{train subnet locally}
  \ENDFOR
  \STATE $W^{t+1} = \frac{\sum_{k \in \kappa_t} \frac{n_k}{n}.w^{t+1}_{k}}{\sum_{k \in \kappa_t}|w^{t+1}_{k}|}$ \algorithmiccomment{cardinal averaging of subnet weights onto supernet}
 % \STATE $W^{0} \leftarrow$ zeros($W_{t}$) \algorithmiccomment{shared-param avg by overlap cardinality}
 % \STATE $W_{sum}  \leftarrow \sum_{k\in S_t} n_k*\mathcal{M}(W^{0},\;arch^{k}_t ,\;w^{k}_{t+1})$
 % \STATE $W_{sum} \leftarrow $  replace\_zeros($W_{sum}$, $W_t$) %
 % \STATE $W_{cnt} \leftarrow \sum_{k\in S_t} \mathcal{M}(W^{0}, arch^{k}_t , n_k*ones(w^{k}_{t+1}))$
 % \STATE $W_{cnt} \leftarrow $  replace\_zeros($W_{cnt}$, $1$) %
 % \STATE $W_{t+1} \leftarrow \frac{W_{sum}}{W_{cnt}}$
\ENDFOR
\end{algorithmic}
\end{algorithm}
% \vspace{-0.1in}




==> tabs/CIFAR10Alpha.tex <==
\begin{table}[tb]
\centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Billion MAC Range}&\multirow{2}{*}{Method}&\multicolumn{3}{c}{Test Accuracy (\%)}\vline\\ \cline{3-5}
        &&$\alpha=100$ & $\alpha=1$ & $\alpha=0.1$ \\ \hline
        \multirow{4}{*}{0.45-0.95}
            &FedAvg&$85.25\pm0.46$&$83.42\pm 0.19$&$77.15\pm 2.5$\\
            &FedNAS&$77.33\pm 0.31$&$71.38\pm 0.37$&$51.57\pm 3.32$\\
            &FedPNAS&$88.83\pm 0.5$&$85.7\pm 0.4$&$78.73\pm 0.45$\\
            &\proposedfed &$\pmb{89.42\pm 0.11}$&$\pmb{88.69\pm 0.2}$&$\pmb{81.81\pm 1.59}$\\ \hline
        \multirow{3}{*}{0.95-1.45}
            &FedAvg&$86.36\pm 0.22$&$84.65\pm 0.11$&$77.99\pm 1.6$\\
            &FedPNAS&$89.27\pm 0.51$&$87.53\pm 0.32$&$81.13\pm 0.4$\\
            &\proposedfed&$\pmb{90.22\pm 0.31}$&$\pmb{89.3\pm 0.35}$& $\pmb{83.27\pm 1.28}$\\ \hline
        \multirow{3}{*}{1.45-2.45}
            &FedAvg&$87.59\pm 0.27$&$86.14\pm 0.23$&$79.93\pm 1.34$\\
            &FedNAS&$86.41\pm 0.1$&$82.13\pm 0.65$&$65.03\pm 2.57$\\
            &\proposedfed&$\pmb{90.93\pm 0.23}$&$\pmb{90.36\pm 0.21}$&$\pmb{84.1\pm 1.71}$\\ \hline
        \multirow{3}{*}{2.45-3.75}
            &FedAvg&$89.44\pm0.67$&$87.88\pm 0.7$&$81.24\pm 1.99$\\
            &FedNAS&$89.43\pm 0.36$&$85.85\pm 0.35$&$68.13\pm 5.04$\\
            &\proposedfed&$\pmb{91.34\pm 0.3}$&$\pmb{90.91\pm 0.15}$&$\pmb{84.72\pm 1.78}$\\ \hline
    \end{tabular}
    \caption{Comparison of \proposedfed with FedAvg and FL NAS methods on CIFAR10 across varying degrees of dataset partition heterogeneity: $\alpha=$ 100, 1 and 0.1}
    \label{tab:NAS_comparison_alphas}
\end{table}

==> tabs/DatasetAblation.tex <==
\begin{table}[tb]
\centering
\footnotesize
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Billion MACs}&\multirow{2}{*}{Method}&\multicolumn{3}{c}{Test Accuracy (\%)}\vline\\ \cline{3-5}
        &&CIFAR10 & CIFAR100 & CINIC10 \\ \hline
        \multirow{4}{*}{0.45-0.95}
            &FedAvg&$85.25\pm0.46$&$43.19\pm 0.54$&$61.76\pm 0.78$\\
            &FedNAS&$77.33\pm 0.31$&$40.92\pm 2.21$&$58.15\pm 0.18$\\
            &FedPNAS&$88.83\pm 0.5$&$45.77\pm 0.68$&$64.3\pm 0.98$\\
            &\proposedfed&$\pmb{89.42\pm 0.11}$&$\pmb{56.35\pm 0.3}$&$\pmb{73.12\pm 0.77}$\\ \hline
        \multirow{3}{*}{0.95-1.45}
            &FedAvg&$86.36\pm 0.22$&$43.92\pm 0.57$&$63\pm 0.17$\\
            &FedPNAS&$89.27\pm 0.51$&$47.8\pm 26$&$66.74\pm 0.32$\\
            &\proposedfed&$\pmb{90.22\pm 0.31}$&$\pmb{57.16\pm 0.23}$& $\pmb{74.5\pm 0.74}$\\ \hline
        \multirow{3}{*}{1.45-2.45}
            &FedAvg&$87.59\pm 0.27$&$44.4\pm 0.56$&$64\pm 0.07$\\
            &FedNAS&$86.41\pm 0.1$&$55.82\pm 0.29$&$69.97\pm 0.27$\\
            &\proposedfed&$\pmb{90.93\pm 0.23}$&$\pmb{57.85\pm 0.31}$& $\pmb{75.08\pm 0.7}$\\ \hline
        \multirow{3}{*}{2.45-3.75}
            &FedAvg&$89.44\pm0.67$&$45\pm 0.27$&$66.02\pm 0.13$\\
            &FedNAS&$89.43\pm 0.36$&$58.39\pm 0.23$&$71.93\pm 0.13$\\
            &\proposedfed&$\pmb{91.34\pm 0.3}$&$\pmb{58.25\pm 0.39}$&$\pmb{75.38\pm 0.73}$\\ \hline
    \end{tabular}
    \caption{ \footnotesize Comparison of \proposedfed with FedAvg and FL NAS methods with data partition heterogeneity $\alpha=100$ across varying datasets: CIFAR10, CIFAR100 and CINIC10}
    \label{tab:NAS_comparison_image_dataset}
\end{table}


==> tabs/ParticipationRatioAblation.tex <==
\begin{table}[]
    \begin{tabular}{|c|c|c|c|}
        \hline
        \multirow{2}{*}{Billion MAC Range}&\multirow{2}{*}{Method}&\multicolumn{2}{c}{Test Accuracy (\%)}\vline\\ \cline{3-4}
        &&C=0.2 & C=0.4 \\ \hline
        \multirow{4}{*}{0.45-0.95}
            &FedAvg&$85.59\pm 0.59$&$85.25\pm0.46$\\
            &FedNAS&$76.23\pm 0.5$&$77.33\pm 0.31$\\
            &FedPNAS&$86.63\pm 0.51$&$88.83\pm 0.5$\\
            &\proposedfed&$\pmb{89.58\pm 0.5}$&$\pmb{89.42\pm 0.11}$\\ \hline
        \multirow{3}{*}{0.95-1.45}
            &FedAvg&$87.01\pm 0.24$&$86.36\pm 0.22$\\
            &FedPNAS&$87.83\pm 0.21$&$89.27\pm 0.51$\\
            &\proposedfed&$\pmb{89.95\pm 0.57}$&$\pmb{90.22\pm 0.31}$\\ \hline
        \multirow{3}{*}{1.45-2.45}
            &FedAvg&$88.04\pm 0.31$&$87.59\pm 0.27$\\
            &FedNAS&$84.65\pm 0.14$&$86.41\pm 0.1$\\
            &\proposedfed&$\pmb{90.7\pm 0.48}$&$\pmb{90.93\pm 0.23}$\\ \hline
        \multirow{3}{*}{2.45-3.75}
            &FedAvg&$89.96\pm 0.65$&$89.44\pm0.67$\\
            &FedNAS&$88\pm 0.38$&$89.43\pm 0.36$\\
            &\proposedfed&$\pmb{91.16\pm 0.45}$&$\pmb{91.34\pm 0.3}$\\ \hline
    \end{tabular}
    \caption{Comparison of \proposedfed with FedAvg and FL NAS methods with data partition heterogeneity $\alpha=100$ across varying client participation ratios: $C=$ 0.2, 0.4}
    \label{tab:NAS_comparison_client_participation}
\end{table}

==> tabs/Shakespeare.tex <==
\begin{table}[tb]
\centering
    \begin{tabular}{|c|c|c|}
        \hline
        Million MAC Range&Method& Test Accuracy (\%)\\ \hline
        \multirow{2}{*}{0-0.5}&FedAvg&$48.52\pm 0.01$\\
            &\proposedfed&$48.22\pm0.27$\\ \hline
        \multirow{2}{*}{0.5-1}&FedAvg&$49.16\pm 0.01$\\
            &\proposedfed&$\pmb{49.81\pm0.16}$\\ \hline
        \multirow{2}{*}{1-1.5}&FedAvg&$51.97\pm 0.03$\\
            &\proposedfed&$\pmb{53.26\pm0.06}$\\ \hline
        \multirow{2}{*}{1.5-2.75}&FedAvg&$53.54\pm 0.11$\\
            &\proposedfed&$\pmb{54.5\pm0.15}$\\ \hline
        \multirow{2}{*}{2.75-4.0}&FedAvg&$53.62\pm 0.1$\\
            &\proposedfed&$\pmb{54.61\pm0.13}$\\ \hline
    \end{tabular}
    \caption{Comparison of \proposedfed with FedAvg on Shakespeare next word prediction text dataset (part of the LEAF benchmark).}
    \label{tab:Shakespeare_dataset}
\end{table}
